SUFFICIENT: A scan-specific unsupervised deep learning framework for high-resolution 3D isotropic fetal brain MRI reconstruction

High-quality 3D fetal brain MRI reconstruction from motion-corrupted 2D slices is crucial for clinical diagnosis. Reliable slice-to-volume registration (SVR)-based motion correction and super-resolution reconstruction (SRR) methods are essential. Deep learning (DL) has demonstrated potential in enhancing SVR and SRR when compared to conventional methods. However, it requires large-scale external training datasets, which are difficult to obtain for clinical fetal MRI. To address this issue, we propose an unsupervised iterative SVR-SRR framework for isotropic HR volume reconstruction. Specifically, SVR is formulated as a function mapping a 2D slice and a 3D target volume to a rigid transformation matrix, which aligns the slice to the underlying location in the target volume. The function is parameterized by a convolutional neural network, which is trained by minimizing the difference between the volume slicing at the predicted position and the input slice. In SRR, a decoding network embedded within a deep image prior framework is incorporated with a comprehensive image degradation model to produce the high-resolution (HR) volume. The deep image prior framework offers a local consistency prior to guide the reconstruction of HR volumes. By performing a forward degradation model, the HR volume is optimized by minimizing loss between predicted slices and the observed slices. Comprehensive experiments conducted on large-magnitude motion-corrupted simulation data and clinical data demonstrate the superior performance of the proposed framework over state-of-the-art fetal brain reconstruction frameworks.

==> LaTeX/table/table_ablation.tex <==
\begin{table}
        \centering

        \caption{ Mean Values of PSNR and SSIM for Different Ablated Models on the Simulated Fetal Brain Datasets.}
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{l|ll}
        \hline
        Methods               & PSNR       & SSIM      \\ \hline
        full model            & 32.02 ± 1.62 & 0.98 ± 0.01  \\
        w/o intensity scale   & 30.04 ± 3.51 & 0.97 ± 0.01 \\
        w/o outlier rejection & 27.76 ± 1.84 & 0.95 ± 0.02 \\
        w/o PSF               & 28.68 ± 0.86 & 0.96 ± 0.01 \\
        w/o SVR-net           & 18.90 ± 0.91 & 0.82 ± 0.04 \\
        w/o SRR-net           & 18.31 ± 1.76 & 0.87 ± 0.02 \\ \hline
        \end{tabular}}
        \label{table_ablation}
        \end{table}

==> LaTeX/table/table_groupA.tex <==
\begin{table}[]
\centering
\caption{ The statistical results of quantitative metrics produced by different methods on the Group A dataset (mean $\pm$ standard deviation). }
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccccc}
\hline
Methods                          & $\operatorname{PSNR} \uparrow$ & $\operatorname{RMSE} \downarrow$ & $\operatorname{SSIM} \uparrow $ & $\mathrm{NCC} \uparrow$ & $\mathrm{NMI} \uparrow$ \\ \hline
SVRTK                            & $18.22 \pm 2.91$               & $0.1289 \pm 0.0386$              & $0.6584 \pm 0.1645$                        & $0.7951 \pm 0.0988$     & $1.1295 \pm 0.0773$     \\
NiftyMIC                         & $19.46 \pm 4.77$               & $0.1210 \pm 0.0585$              & $0.7908 \pm 0.1430$                        & $0.8613 \pm 0.1057$     & $1.1802 \pm 0.1007$     \\
$\mathrm{NeSVoR}$                & $21.28 \pm 4.66$               & $0.0981 \pm 0.0503$              & $0.8507 \pm 0.0983$                        & $0.9287 \pm 0.0439$     & $1.2296 \pm 0.0951$     \\
$\mathrm{SVoRT}+\mathrm{NeSVoR}$ & $22.09 \pm 4.41$               & $0.0875 \pm 0.0375$              & $0.8636 \pm 0.0768$                        & $0.9288 \pm 0.0453$     & $1.2302 \pm 0.0959$     \\
SUFFICIENT                       & $\bold{24.25 \pm 3.22}$               & $\bold{0.0651 \pm 0.0220}$              & $\bold{0.8909 \pm 0.0433}$                        & $\bold{0.9529 \pm 0.0256}$     & $\bold{1.2151 \pm 0.0806}$     \\ \hline
\end{tabular}}
\label{table_groupA}
\end{table}

==> LaTeX/table/table_groupB.tex <==
\begin{table}[]
\centering
\caption{ The mean values of the quantitative metrics produced by different methods on the Group B dataset.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccccc}
\hline
Methods      & $\operatorname{PSNR} \uparrow$ & RMSE $\downarrow$   & $\operatorname{SSIM} \uparrow$ & $\mathrm{NCC} \uparrow \longleftarrow$ & $\mathrm{NMI} \uparrow$ \\ \hline
SVRTK        & $16.86 \pm 1.75$               & $0.1463 \pm 0.0286$ & $0.4850 \pm 0.1160$            & $0.7430 \pm 0.0955$                    & $1.1108 \pm 0.0668$     \\
NiftyMIC     & $15.63 \pm 4.14$               & $0.1819 \pm 0.0742$ & $0.5757 \pm 0.2327$            & $0.6300 \pm 0.2219$                    & $1.1081 \pm 0.0900$     \\
NeSVoR       & $19.21 \pm 4.03$               & $0.1196 \pm 0.0464$ & $0.8174 \pm 0.1063$            & $0.8848 \pm 0.0833$                    & $1.2092 \pm 0.1066$     \\
SVoRT+NeSVoR & $20.99 \pm 4.62$               & $0.1001 \pm 0.0444$ & $0.8492 \pm 0.0853$            & $0.9125 \pm 0.0625$                    & $1.2247 \pm 0.1007$     \\
SUFFICIENT   & $\bold{23.39 \pm 2.87}$               & $\bold{0.0709 \pm 0.0212}$ & $\bold{0.8810 \pm 0.0476}$            & $\bold{0.9478 \pm 0.0266}$                    & $\bold{1.2073 \pm 0.0802}$     \\ \hline
\end{tabular}}
\label{table_groupB}
\end{table}



==> LaTeX/table/table_groupC.tex <==
\begin{table}[]
\centering
\caption{ The mean values of the quantitative metrics produced by different methods on the Group C dataset.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|ccccc}
\hline
Methods                          & $\operatorname{PSNR} \uparrow$ & $\operatorname{RMSE} \downarrow$ & $\operatorname{SSIM} \uparrow$ & $\mathrm{NCC} \uparrow$ & NMI $\uparrow$       \\ \hline
SVRTK                            & $16.12 \pm 1.68$               & $0.1591 \pm 0.0298$              & $0.4429 \pm 0.0999$            & $0.6841 \pm 0.1247$     & $1.0964 \pm 0.0648$  \\
NiftyMIC                         & $13.74 \pm 3.59$               & $0.2209 \pm 0.0787$              & $0.4617 \pm 0.2735$            & $0.4477 \pm 0.2881$     & $1.0812 \pm 0.0801$  \\
$\mathrm{NeSVoR}$                & $13.18 \pm 3.02$               & $0.2311 \pm 0.0737$              & $0.5198 \pm 0.2416$            & $0.5949 \pm 0.2396$     & $1.1016 \pm 0.0964$  \\
$\mathrm{SVoRT}+\mathrm{NeSVoR}$ & $20.25 \pm 5.46$               & $0.1162 \pm 0.0723$              & $0.7980 \pm 0.1881$            & $0.8515 \pm 0.1970$     & $1.1971 \pm 0.1080$  \\
SUFFICIENT                       & $\bold{22.40 \pm 3.28}$               & $\bold{0.0807 \pm 0.0272}$              & $\bold{0.8718 \pm 0.0594}$            & $\bold{0.9333 \pm 0.0397}$     &  $\bold{1.2055 \pm 0.0843}$ \\ \hline
\end{tabular}}
\label{table_groupC}
\end{table}



==> LaTeX/table/table_simulation_3mm.tex <==
    \begin{table}
    \centering

    \caption{  The statistical results of quantitative metrics produced by different methods on the Group D datasets.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l|lll}
    \hline
    method       & PSNR       & SSIM      & NCC       \\ \hline
    NiftyMIC     & 20.69 ± 1.51 & 0.85 ± 0.06 & 0.81 ± 0.05 \\
    SVRTK        & 23.46 ± 1.43 & 0.90 ± 0.03  & 0.89 ± 0.04 \\
    NeSVoR       & 22.38 ± 2.85 & 0.89 ± 0.06 & 0.87 ± 0.05 \\
    SVoRT+NeSVoR & 30.30 ± 1.74  & 0.97 ± 0.02 & 0.97 ± 0.02 \\
    SUFFICIENT   & 32.02 ± 1.61      & 0.98 ± 0.01 & 0.98 ± 0.01 \\ \hline
    \end{tabular}
    \label{simulation_3mm_table}}
    \end{table}
